SRL: Scaling Distributed Reinforcement Learning to Over Ten Thousand Cores

The ever-growing complexity of reinforcement learning (RL) tasks demands a distributed system to efficiently generate and process a massive amount of data. However, existing open-source libraries suffer from various limitations, which impede their practical use in challenging scenarios where large-scale training is necessary. In this paper, we present a novel abstraction on the dataflows of RL training, which unifies diverse RL training applications into a general framework. Following this abstraction, we develop a scalable, efficient, and extensible distributed RL system called ReaLlyScalableRL, which allows efficient and massively parallelized training and easy development of customized algorithms. Our evaluation shows that SRL outperforms existing academic libraries, reaching at most 21x higher training throughput in a distributed setting. On learning performance, beyond performing and scaling well on common RL benchmarks with different RL algorithms, SRL can reproduce the same solution in the challenging hide-and-seek environment as reported by OpenAI with up to 5x speedup in wall-clock time. Notably, SRL is the first in the academic community to perform RL experiments at a large scale with over 15k CPU cores. SRL source code is available at: https://github.com/openpsi-project/srl .

==> main/archived.tex <==
\hzcmt{\textbf{An Alternative Outline:}} \\

\hz{\texttt{para.1}: The importance of *large-scale* RL systems (better mention
some data processing applications to fit SIGMOD)} \\

\hz{\texttt{para.2}: The (unique) characteristics of RL, including the different
roles in the system: environment simulator, decision maker? trainer} \\

\hz{\texttt{para.3, 4, maybe 5}: Existing RL systems/libraries struggle to scale to
industrial sizes (e.g., $>1000$ CPU cores). The problems are:}
\hzcmt{The current text is not quite clear on this}
\begin{itemize}
\item \hz{Trainer too slow? Why?}
\item \hz{The separation of inference and simulation on different cores/machines
causes resource waste and extra network traffic. What's the scalability bottleneck then?}
\item \hz{Diversity of environments? How does this affect scalability?}
\end{itemize} \\

\mzy{Trainer too slow: not enough sample throughput due to single-threaded trainer implementation and data transmission speed (for example, ray.get() is too slow in the example of RLlib) \\
\indent Scalability bottleneck: due to the fact that rollout workers can be easily parallelized infinitely, the bottleneck is usually on trainers (network throughput, GPU utilization, DDP synchronization...) However, depending on how many resources (GPU, CPU, memory) there are in the cluster, bottleneck can also be the number of CPU or memory resources. \\
\indent Environment diversity: Depending on environment rollout speed, the ratio of GPU and CPU (or memory) needed to optimize FPS is different. It seems it does not affect scalability directly, but I think it may be something worth mentioning?}



\hz{\texttt{para.6}: Other engineering and usability challenges.} \\

\hz{\texttt{para.7, maybe 8}: A brief introduction to our system. Focus on how we solve
the above issues. Worker-based abstraction?}
\hzcmt{We need a name for our system.}\\

\hz{\texttt{para.9}: A brief summary of experimental results.} \\

\hz{\texttt{para.10}: Contributions.} \\
\begin{itemize}
\item \hz{new architecture to build scalable RL systems}
\item \hz{An implementation that is fast and easy-to-deploy for a wide-range of RL applications}
\item \hz{Benchmarked the systems under super large scale ()}
\item \hz{Results are impressive. To the best of our knowledge, xxx is the first system that can
scale to 10000+ CPUs and 100+ GPUs.}
\end{itemize}

\hzcmt{A lot of the text in the current intro (especially those introducing general RL)
can be moved to the background section.}



\subsection{per-paragraph outlines}
\subsubsection{para 1}
\begin{itemize}
    \item Reinforcement learning (RL) is a trending solution to many complicated tasks. (Importance of RL)
    \item The problem that single-machine RL usually costs weeks to finish a task could be solved by distributed RL. (Importance of distributed RL)
    \item Distributed RL is a emerging demand. (Examples: AlphaGo, OpenAI5, AlphaStar)
\end{itemize}

\subsubsection{para 2}
\begin{itemize}
    \item To enable distributed deep reinforcement learning, researchers have made great efforts on developing distributed deep RL algorithms. (Introduction to distributed RL algorithms)
    \item To run such distributed RL algorithms, the architecture must preserve the ability to simulate the environments, train the models, and use the model to instruct agents to act in the environments. (Basic requirements for RL systems, different roles in RL systems)
\end{itemize}


\subsubsection{para 3: challenges}
\begin{itemize}
    \item The system needs to be compatible for all algorithms and all environments.
    \item Although environments rollouts can be parallelized naturally, and trainers can be scaled due to distributed deep learning, RL system are hard to scale linearly because of:
    \begin{itemize}
        \item underlying dataflow requires an enormous amount of network bandwidth
        \item Due to different resources configuration, computational bottleneck could be various.
        \item Limitations of distributed deep learning.
    \end{itemize}
\end{itemize}

\subsubsection{para 4 (or 5): existing systems}
\begin{itemize}
    \item \cite{gorila} is the first massively distributed architecture for deep reinforcement learning. The architecture is specially designed for distributed version of deep RL algorithm DQN, and it is only applied to games from atari. 
    \item Later, many proposed methods to run distributed reinforcement learning efficiently, with both new algorithms along with architectures (designed for them) (\cite{a3c}; \cite{apex}; \cite{impala}; \cite{dppo}; \cite{ddppo}; \cite{tfagents}).
    \item There are also re-implementations for algorithms such as \cite{impala}, aiming to improve the performance or scale up without changing original algorithm design. (\cite{torchbeast}; \cite{seedrl}) \cite{surreal} is a distributed reinforcement learning framework focused on algorithms with continuous control.
    \item Some of the existing systems were research frameworks for academic use, aiming to provide an easy-to-implement platform for new algorithms. (\cite{dopamine}; \cite{acme}).
    \item For distributed applications of reinforcement learning, \cite{Ray} and \cite{Fiber} provided generic primitives for distributed computations, and built distributed RL frameworks based on the primitives (\cite{rllib}).
    \item  \cite{rllib} is a open-source reinforcement library which support scalable rollout and training. 
    \begin{itemize}
        \item  RLLib includes various algorithms and is able to run them in a distributed fashion. 
        \item  RLLib merged different architectures for algorithms into several components (rollout workers, trainers), and controlled them in a hierarchical way.
        \item Due to RLLib's hierarchical control and underlying communication using ray, there exists unnecessary overhead that harms the final performance.
        \item RLLib did not support scalable GPU inference.
    \end{itemize}
\end{itemize}

\subsubsection{para 6: other challenges}
\begin{itemize}
    \item The users should be able to develop new algorithms easily. Implementing new algorithms in current open-source systems (or frameworks) requires a lot of coding because the abstractions of RL workloads are not generalized enough.
    \item Some RL tasks needs agent-policy mapping, which requires flexible underlying data streams. Flexible data streams also benefits resource allocation. 
\end{itemize}

\subsubsection{para 7, 8: introduction to our system}
\begin{itemize}
    \item We designed a general architecture (actor, policy, trainer worker ...) that support popular RL algorithms and enable users to design new algorithm within the architecture easily. 
    \item We proposed a worker-based programming model to implement our system, and support users to implement new algorithms and  components with minimum coding. 
    \item We designed and reorganized data streams between aforementioned components to achieve effectiveness, maximize the throughput, and solve policy-agent mapping problem at the same time.
    \item We analysed each part of reinforcement learning workloads in detail, and proposed solutions to optimize their performance respectively. 
    \begin{itemize}
        \item We implemented threaded trainers, and maximized trainer throughput.
        \item We implemented double-buffering (sample factory) with env-ring to maximize environment rollout efficiency.
        \item We provided GPU inference support and analysed in which condition GPU inference is better than CPU inference.
    \end{itemize}
    \item In conclusion: Following the principles and methods we discovered and proposed, 
    we built (sysname), a scalable reinforcement learning system with high efficiency. We implemented the system using the worker-based model we proposed, saving lots of unnecessary coding and enabling fast and simple development for new algorithms. 
\end{itemize}

\subsubsection{para 9: experiment results}
\todo{modify after a100 experiments and small experiments}
\begin{itemize}
    \item 
\end{itemize}


\subsubsection{para 10: contributions}
In summary, we list our contribution as follows.
\begin{itemize}
    \item We analysed how to improve performance for RL tasks, and proposed several solutions to existing obstacles. Furthermore, we conducted a series of experiments to show that the solutions are viable.
    \item We built a scalable reinforcement learning system (sysname) according to our findings, with a novel architecture that enabled scalability and efficient resource usage. 
    \item We proposed a worker-based programming model to implement (sysname), which is fast and easy-to-deploy for a wide range of RL applications.
    \item We conducted large scale experiments of training tasks on academic environments, with popular RL algorithms to benchmark the performance of (sysname). In total, 10000+ CPUs and 100+ GPUs are deployed in the largest-scale experiment. The results showed that acceleration by piling up resources was almost linear until reaching the limitation of \texttt{pytorch} DDP. To the best of our knowledge, (sysname) is the first system that can achieve this result. 
\end{itemize}

%\hz{\texttt{para.10}: Contributions.} \\
%\begin{itemize}
%\item \hz{new architecture to build scalable RL systems}
%\item \hz{An implementation that is fast and easy-to-deploy for a wide-range of RL applications}
%\item \hz{Benchmarked the systems under super large scale ()}
%\item \hz{Results are impressive. To the best of our knowledge, xxx is the first system that can
%scale to 10000+ CPUs and 100+ GPUs.}
%\end{itemize}

%\hzcmt{A lot of the text in the current intro (especially those introducing general RL)
%can be moved to the background section.}



\subsubsection{para 1: intro to RL components}
\begin{itemize}
    \item RL agents adjust their policies according to observations and rewards in the simulated environments.
    \item A reinforcement learning system has following critical components
    \begin{itemize}
        \item actors that simulate and act in the environments.
        \item policies that decides how the actors behave
        \item trainers (algorithms) that update the policy
    \end{itemize}
\end{itemize}

\subsubsection{para 2: actors}
\begin{itemize}
    \item Environment simulators are usually software and scripts provided by academic community or commercial companies. 
    \item Actors interact with environment simulator, to generate experiences for training. Experiences are composed of observations, states and actions.
    \item There exists a standard API for RL environments named \textbf{gym}, which is commonly used by academic reinforcement learning community.
\end{itemize}

\subsubsection{para 3: policy}
\begin{itemize}
    \item To control the agents in the simulation environments, a decision making process is necessary.
    \item A model completes its inference (also known as forward propagation) in either GPU or CPU devices.
    \item The inputs are observations and states received from environment simulation and the output are actions, which instruct agents in environments.
\end{itemize}

\subsubsection{para 4: trainers}
\begin{itemize}
    \item Trainers receive experiences from actors and exploit them to update the model.
    \item Trainers can be parallelized with distributed deep learning techniques, such as pytorch DDP.
    \item The bottleneck of the entire system usually lies on trainers when CPU resources are sufficient. The reason is that the number of parallel environment simulators could increase infinitely.
\end{itemize}

\subsubsection{para 5: underlying data streams}
\begin{itemize}
    \item In a reinforcement learning system, data streams could be enormous and complex.
    \item The data streams could be enormous because the actors can be parallelized infinitely and generate a large amount of experiences for training in a short time.
    \item The data streams could be complex, because agents sometimes needs to follow different policies, and different policies might be trained in different trainers. There are mappings between actors, policies and trainers, which requires data streams to maintain these mapping relationships.
\end{itemize}

\subsubsection{para 6: other components}
\begin{itemize}
    \item Some reinforcement learning algorithms require buffers for experiences
    \item Parameter servers updates model from trainers, and to policies. Since currently most models for deep reinforcement learning is not large in size, parameter servers are usually not bottlenecks in a reinforcement learning system.
\end{itemize}


\subsection{Goals}
\subsubsection{para 1}
\begin{itemize}
    \item The most fundamental goal of optimizing a reinforcement learning system is to train agents faster with certain amount of resources.
    \item To pursuit training efficiency, we can either improve algorithms to reach better sample efficiency (which is not inside the scope of our paper), or improve efficiency to generate and consume samples with our limited resources. 
    \item To reduce training time, sample throughput for trainers is a critical target to optimize.
    \todo{Async training and sync training?}
    \item The final sample throughput is decided by two major factors.
    \begin{itemize}
        \item The first one is how much experiences actors can generate. (para 2)
        \item The second one is how much data can trainers exploit to train. (para 3)
    \end{itemize}
\end{itemize}

% actors and inference
\subsubsection{para 2}
\begin{itemize}
    \item The actors can be easily paralellized when resources are sufficient. However, this is not always the case. It is meaningful to improve the performance of actors to generate experiences faster.
    \item The environment simulators are usually external software that execute with actors. It is not practical to optimize time cost of each simulation step. 
    \item The main optimization goal is to optimize inference efficiency.
    \item Model inference can be performed on both GPU and CPU. GPU inference is faster on computation, but inter-nodes communication could be a overhead.
    \item Our insight is that to overlap environment simulation steps and inference steps to reduce resource idle time to the minimum (\cite{samplefactory})
\end{itemize}

% training
\subsubsection{para 3}
\begin{itemize}
    \item There are two major factors that could decides sample throughput for trainers. The first one is that how fast can trainer consume samples from rollout workers. The second one is how much samples can be used by GPUs to optimize model in a certain time. 
    \item To improve two criteria above, parallelizing training with multiple GPUs is crucial. 
\end{itemize}

\subsubsection{para 4}
There are also other goals for RL system.
\begin{itemize}
    \item Implementation of current popular RL algorithms
    \item Easy to implement new algorithms under the framework
    \item Easy to schedule, configure and run experiments
\end{itemize}


\subsubsection{para 1}
% generally introduce the system architecture
\todo{figure to show basic architecture: workers, streams, controller}
\begin{itemize}
    \item As section \ref{subsec:intro2rl} described, deep reinforcement learning workloads typically  includes simulation, policy inference and training.
    \item These common workloads can be summarized with two simple patterns: computation to generate data and data transmission. Separating two kinds of workloads can simplify implementation, and help with performance optimization.
    \item With such insights, we designed a worker-based programming model to modularize the components and simplify the implementation (Section \ref{subsec:workerbased}). The worker-based programming model is separated into workers that deal with computation workloads, and data streams that are in charge of data transmission between workers.
    \item Figure XX shows a basic structure of worker-based programming model.
\end{itemize}

\subsubsection{para 2}
\begin{itemize}
    \item With worker-based programming model, we implemented several components to support most of the state-of-the-art deep reinforcement learning algorithms. 
    \item  Common workers are actor workers, policy workers, and trainer workers (Section \ref{subsec:workers}). For storage requirement in some algorithm, we also implemented buffer workers.
    \item For basic RL data transmission, we implemented inference stream and sample stream (Section \ref{subsec:streams}). Inference streams communicate actor workers and policy workers. Sample streams deal with data transmission between actor workers (or policy workers) and trainers.
\end{itemize}

\subsubsection{para 3}
\begin{itemize}
    \item To manage workers, we implemented a centralized controller. The controller submits experiments, handles resource requests, and tells workers when to start or terminate.
    \item We also implemented a parameter server on an NFS for model storage and updates.
\end{itemize}

\begin{table*}[h]
    \centering
    \begin{tabular}{ |c|c|c|c| } 
     \hline
      & Computation & Input & Output \\
     \hline
     Simulator & Environment simulation & actions & observations \\ 
     \hline
     Policy Inference & Model inference & O, M & A \\
     \hline
     Training & Model training & A, O & M \\
     \hline
    \end{tabular}
    \caption{Common RL workloads, A: actions, O: observations and states, M: model updates}
    \label{tab:rlworkload}
\end{table*}

\subsection{Worker-based programming model}
\label{subsec:workerbased}
\subsubsection{para 1:}
\begin{itemize}
    \item Insight: Simulation, policy inference and training and other tasks in reinforcement learning usually can be concluded with a pattern of two kinds of operations: computation and data transmission. (\ref{tab:rlworkload})

    
    
    \item We designed a worker-based programming model that modularizes reinforcement learning workloads, and simplify implementations of the system. 
    \item Corresponding to two patterns, there are two parts for the programming model: workers and data streams.
    \item Workers are in charge of computation, and have interface for data streams for input and output of computation. 
    \item Data streams usually exchange large amount of data between workers. They support large throughput, efficient data transmission. We do not use data streams for operations that do not usually become bottlenecks, such as model updates and communication between controllers and workers.
\end{itemize}

% about implementing new algorithm and workers, to be discussed
\subsubsection{para 2:}
\begin{itemize}
    \item Worker-based programming model make implementing algorithms more simple. It keeps the complexity of underlying communication between workers from reinforcement learning researchers.
    \item If users intend to add new computations into algorithm pipeline, they only need to implement a new worker class and define its communication by creating data streams.
\end{itemize}

% expressiveness
    
\subsubsection{Workers}
\label{subsec:workers}

\subsubsection{para 1:}
\begin{itemize}
    \item We implemented several kinds of workers to support basic deep reinforcement learning tasks: actor workers for environment simulation, policy workers for model inference, and trainer workers for training. There are also other workers for optional requirements, for example, buffer workers for experience buffering.
    \item As python codes in Listing \ref{lst:worker} show, workers run in a loop performing \texttt{self.poll()} at every step.
    \item \texttt{self.poll()} defines computation workloads for a worker. For example, if the worker simulates environments, it should execute \texttt{env.step()} inside \texttt{self.poll()}. For a trainer, it should execute one training step inside \texttt{self.poll()}.
    \item The implementation of workers varies because of different requirements for computational workloads. In the remaining part of the section, we will introduce details for actor, policy, and trainer workers.
\end{itemize}

\subsubsection{para 2: actor workers and policy workers}
\begin{itemize}
    \item Actor workers simulate environments, which usually need to run external software on various platforms. 
    \item With enough resources, actor workers could be heavily parallelized, and generate large amount of data. 
    \item Policy workers responds actor workers' inference requests with actions. To keep models in policy workers up-to-date, policy workers also needs to pull parameters from parameter servers once in a while.  
    \item Policy workers could run the computation on both CPU and GPU devices (which will be discussed in detail in section 4 (ref)).
    \item Actor workers and policy workers run together to generate experiences (consist of actions, observations and states) as training data. 
\end{itemize}

\subsubsection{para 3: trainer workers}
\begin{itemize}
    \item Trainer workers receive experiences from actor and policy workers, using deep learning to update model parameters. 
    \item To fully utilize GPU resources on trainer workers, trainer workers need to consume large batches of experiences in a short time. This makes trainer workers are usually bottlenecks in the entire system (discuss in detail in section 4 (ref)).
    \item When running asynchronous algorithms, to overlap data consuming and training, GPU computation is finished on a independent thread. 
    \item Different from existing systems, \sysname comes with a multi-trainer design. (Advantages of multi-trainers, sample throughput, training speed)
\end{itemize}

\subsection{Data streams}
\label{subsec:streams}
\subsubsection{para 1:}
\begin{itemize}
    \item Data streams are components that takes charge in large data transfer. In deep reinforcement learning context, the most common types of large data are training samples (experiences) and inference data (observations and actions).
    \item We implemented two types of data streams in our system: inference stream and sample stream. As the names suggest, inference stream delivers observations and actions, and sample streams delivers training samples.
    \item Difference between inference streams and sample streams: Inference streams are duplex because actor workers and policy workers exchange observations and actions. Sample streams are simplex, because only actor workers send experiences to trainer workers, and trainer workers do not reply.
    \item Throughput for sample streams directly influence training speed, because workers need to consume large batches of experiences in a short time. Therefore it is essential to maximize throughput for sample streams to avoid congestion in sample delivery.
    
\end{itemize}

\subsubsection{para 2:}
\begin{itemize}
    \item In one RL experiment in our system, there might be multiple instances of sample streams and inference streams. Instances of data streams are isolated from each other.
    \item Sometimes for the requirements of certain algorithms, different policies need to be trained in one experiment. This means different actor workers are mapped to different policy workers and different trainer workers. With such requirement, inference streams and sample streams establish transmission between certain groups of workers to maintain an actor-policy mapping.
\end{itemize}

\subsubsection{para 3: implementation }
\begin{itemize}
    \item When configuring experiments, we assign a name for each data stream we intend to use. 
    \item If we want to connect a worker to some data stream, we specify the name in worker configuration to establish connection.
    \item After configuration, each data stream will establish connection between workers, with basic ZeroMQ (cite zeromq) communication patterns.
    \item ZeroMQ is a networking library with equivalent performance to lower level protocols. Our data stream implementation adds no overhead after launching the experiments. As a results, our data stream is able to reach transmission speed comparable to underlying communication protocols.
\end{itemize}

\subsection{Infrastructure}
\subsubsection{para 1:}
\begin{itemize}
    \item To manage the life cycle of workers and data streams, we designed and implemented a centralized controller. 
    \item The controller reads configurations, allocates resources to workers, and establishes communication between workers by initializing data streams.
    \item Essentially, the controller is a RPC client that sends requests to servers (workers) to manage the life and death of a worker process.
    \item We use \texttt{slurm} to manage resources and launch the processes to setup RPC servers.
    
\end{itemize}




\todo{related works to section 6}

The related works could be introduced from 3 parts: 
\begin{itemize}
    \item application (OpenAI5, AlphaGo, AlphaStar) to be evidences of importance of large-scale RL. 
    \item algorithms that supports distributed architecture to show the avalability of large-scale RL.
    \item existing distributed (or non-distributed) RL systems.
\end{itemize}

Detailed outlines: 
\begin{itemize}
    \item Recent years have seen reinforcement learning agents that are able to perform certain tasks with skills that surpass human. (OpenAI5 \cite{openai5}, AlphaStar \cite{alphastar}, AlphaGo \cite{alphago}) To train agents with such complexity efficiently, enormous data set and large-scale computation are crucial. OpenAI5 \cite{openai5} were trained with a custom distributed training platform in OpenAI, utilizing a large-scale of computing resources. Unfortunately, academic community has no access to the design and implementation of OpenAI's distributed training platform.
    \item Gorila \cite{gorila} is the first massively distributed architecture for deep reinforcement learning. The architecture is specially designed for distributed version of deep RL algorithm DQN, and it is only applied to games from atari. 
    \item Later, many proposed methods to run distributed reinforcement learning efficiently, with both new algorithms along with architectures (designed for them) (A3C\cite{a3c}; Apex \cite{apex}; Impala \cite{impala}; DPPO\cite{dppo}; DDPPO \cite{ddppo}; TF-agents \cite{tfagents}).
    \item There are also re-implementations for algorithms such as Impala \cite{impala}, aiming to improve the performance or scale up without changing original algorithm design. (TorchBeast\cite{torchbeast}; SeedRL\cite{seedrl}) Surreal \cite{surreal} is a distributed reinforcement learning framework focused on algorithms with continuous control.
    \item Some of the existing systems were research frameworks for academic use, aiming to provide an easy-to-implement platform for new algorithms. (Dopamine \cite{dopamine}; Acme \cite{acme}).
    \item For distributed applications of reinforcement learning, Ray \cite{Ray} and Fiber \cite{fiber} provided generic primitives for distributed computations, and built distributed RL frameworks based on the primitives (RLlib \cite{rllib}).
    \item  RLlib \cite{rllib} is a open-source reinforcement library which support scalable rollout and training. 
    \begin{itemize}
        \item  RLLib includes various algorithms and is able to run them in a distributed fashion. 
        \item  RLLib merged different architectures for algorithms into several components (rollout workers, trainers), and controlled them in a hierarchical way.
        \item Due to RLLib's hierarchical control and underlying communication using ray, there exists unnecessary overhead that harms the final performance.
        \item RLLib came with a single-trainer design, which impeded multi-node multi-GPU training for RL.
        \item RLLib did not support scalable GPU inference.
    \end{itemize}
\end{itemize}



%\subsection{Motivation and Goals}
% \subsection{Motivation}
% \label{sec:motivation}


% Recent RL systems have made progress on developing algorithms that can run efficiently on a distributed architecture~\cite{gorila,a3c,ga3c,ClementeMC17, dppo,apex,impala,ddppo}.
% % \todo{cite} 
% However, these algorithms/systems are often ad-hoc, i.e., targeting specific tasks. To support distributed training for a new RL algorithm, %\yw{I don't know if we need to show our system can also support multiple RL algorithms at some point?} 
% one must re-implement the aforementioned core components over and over again. This development inefficiency calls for a general-purpose RL system that can support a wide range of RL scenarios. To meet such needs, a large number of open-source RL libraries and frameworks have been proposed over these years \cite{tfagents,rllib,horizon,dopamine,surreal,torchbeast,seedrl, samplefactory,rlpyt2019Adam}.

% There are two optimization directions to improve the training efficiency in an RL system. The first is to improve the sample efficiency of a specific RL algorithm, which is out of the scope of this paper. In this paper, we focus on the second direction, which is to improve the training speed so that the system can complete more training iterations with larger training batch sizes within the same amount of wall clock time. A good measure for this is the sample throughput for the trainers. To achieve a high trainer throughput, it requires that (1) actors generate data samples quickly, and (2) trainers consume samples in a speed that keeps up with the sample generation. 

% Simulation can be easily parallelized with abundant compute resources. Environments or simulators are typically black-box external programs. It is usually impractical to optimize the time cost of each simulation step. Another factor that influences sample generation time is policy inference. As mentioned in section \ref{subsec:rlsystem}, policy inference can be done in both GPU and CPU devices. Evidently, computing forward propagation in GPUs takes less time than doing so in CPUs. When policy models are complex, in spite of communication overheads, GPU inference improves sample generation speed greatly. However, few systems or libraries support batched inference on GPUs. This is because in traditional designs, simulation and policy inference are coupled tightly in actors. To enable GPU accelerated inferences, each actor must store a copy of policy neural network into a corresponding GPU, which leads to a huge waste of GPU memories. This prevents prior systems from paralleling their actors massively when using GPU-accelerated inference. We, therefore, propose a system architecture that decouples simulation and policy inference in \sysname.

% Each trainer has a data buffer that receives samples from actors to consume later for batched training. Parallelizing trainers can not only increase the cumulative bandwidth for the buffers but also speed up each training iteration. Nevertheless, among existing open-source systems, only RLlib \cite{rllib} supports single-node multi-GPU trainers, which handles the scalability bottleneck to a very limited scale. In \sysname, we propose multi-node multi-GPU trainers with multiple buffers, which are synchronized by distributed data parallel (i.e., PyTorch DDP \cite{ddp}). %\hzcmt{heavy rewrite, please check}

% Recent years have seen reinforcement learning agents that are able to perform certain tasks with skills that surpass human specialists \cite{openai5,alphastar,alphago}. To train agents with such complexity and intelligence, countless iterations of simulation and enormous number of training samples are crucial to success. It is impossible to train similar agents within weeks or even months without a distributed reinforcement learning system that is able to run experiments on a large scale. Speeding up RL training has become a increasingly emergent problem for reinforcement learning community. 

% The rest of the paper is organized as follows. In Section~\ref{sec:architecture}, we describe \sysname's system architecture and implementation details. Section~\ref{sec:performance} focuses on performance analysis and optimizations of each system component. We show our experiment results in Section~\ref{sec:exp} followed by a related work discussion in Section~\ref{sec:related}. Finally, we conclude in Section~\ref{sec:conclusion}.

% None of them, however, is able to scale efficiently even with a medium-sized cluster. Most of them only parallelize the tightly-coupled simulation and policy inference without a multi-GPU support for the training, thus making the training a pipeline blocker.

% As a result, there are lots of recent reinforcement learning progresses lean towards distributed algorithms that supports distributed computation, or bases on a distributed architecture \cite{gorila,a3c,apex,dppo,ddppo,tfagents,impala}. However, when researchers develop new RL algorithms, implementations of previous algorithms are always ad-hoc. Researchers always need to re-implement core components of RL training over and over again. The requirement for general RL systems that has the capability to run various algorithms emerges. 

% To meet the needs for RL community, a large number of open-source RL libraries and frameworks have been developed over these years \cite{dopamine,torchbeast,tfagents,surreal,seedrl,rllib,horizon}. However, none of these systems or libraries could be efficiently distributed even on a medium-size cluster. Most of them only simply parallelize environment rollouts. Few supports multi-GPU training across GPU-nodes. The problem of scaling the performance of a reinforcement learning system on a large-size cluster remains unsolved.


% The most fundamental goal of scaling and optimizing a reinforcement learning system is to train agents faster with certain amount of resources. To pursuit training efficiency, we can either improve algorithms to reach better sample efficiency (which is not inside the scope of our paper), or improve efficiency to generate and consume samples with our limited resources. 

% To measure the training speed without peeking into sample efficiency of RL algorithms, sample throughput for trainers is a suitable target to optimize. The final sample throughput for trainers is decided by two major factors. The first one is that how much samples actors can generate within a period of time. The second one is how much data can trainers consume to optimize the policy.


%\hzcmt{consider adding a roadmap paragraph here. e.g., The rest of the paper is organized as follows...}

%\mzy{The rest of this paper is organized as follows: In Section~\ref{sec:architecture}, we introduce the architecture of \sysname in details, and explain why we design \sysname in this way. In Section~\ref{sec:performance}, we analyse \sysname's performance, and show some of the optimizations in the system. In Section~\ref{sec:exp}, we show our experiment details and results. In Section~\ref{sec:related}, we introduce related works to our paper. And finally we make a conclusion in Section~\ref{sec:conclusion}.}

%To improve the sample efficiency of algorithms, trainers are always required to preserve a replay buffer that receives samples from actors, and stores them for trainers to consume. In this case, to improve sample consuming rate for trainers, we need to lower the time cost for each training step, and make buffer receive samples in a higher rate. Both of the problems can be solved by parallelize the trainers. However, in spite of the existence of mature techniques to build data-parallel trainers such as PyTorch DDP \cite{ddp}, only RLlib \cite{rllib} supports single-node multi-GPU trainers. The limited bandwidth of a single endpoint also harms the consuming rate for replay buffers on trainer. 

\iffalse
Apart from total sample throughput, there are other goals that an RL system pursuits such as flexibility. An flexible RL system should allow users to run diverse environments and implement their own algorithms. \hzcmt{this paragraph is very weak. Expand this or get rid of it}.
\fi
%Simulation can be easily parallelized when resources are sufficient. Environments or simulators are typically external programs that serve as black boxes. It is usually not practical to optimize the time cost of each simulation step. Another factor that influences sample generation time is policy inference. As mentioned in section \ref{subsec:rlsystem}, policy inference can be done in both GPU and CPU devices. Evidently, computing forward propagation in GPUs takes less time than doing so in CPUs. When policy models are complex, in spite of communication overheads, GPU inference improves sample generation speed greatly. However, in prior works, few systems or libraries support batched inference on GPUs. This is because in traditional designs, simulation and policy inference are always coupled tightly in actors. To enable GPU accelerated inferences, each actor must store a copy of policy neural network into a corresponding GPU, which leads to a huge waste of GPU memories. This prevent prior systems to parallel their actors massively when using GPU-accelerated inference. 
